Smooth Non-Rigid Shape Matching via Effective Dirichlet Energy Optimization

We introduce pointwise map smoothness via the Dirichlet energy into the functional map pipeline, and propose an algorithm for optimizing it efficiently, which leads to high-quality results in challenging settings. Specifically, we first formulate the Dirichlet energy of the pulled-back shape coordinates, as a way to evaluate smoothness of a pointwise map across discrete surfaces. We then extend the recently proposed discrete solver and show how a strategy based on auxiliary variable reformulation allows us to optimize pointwise map smoothness alongside desirable functional map properties such as bijectivity. This leads to an efficient map refinement strategy that simultaneously improves functional and point-to-point correspondences, obtaining smooth maps even on non-isometric shape pairs. Moreover, we demonstrate that several previously proposed methods for computing smooth maps can be reformulated as variants of our approach, which allows us to compare different formulations in a consistent framework. Finally, we compare these methods both on existing benchmarks and on a new rich dataset that we introduce, which contains non-rigid, non-isometric shape pairs with inter-category and cross-category correspondences. Our work leads to a general framework for optimizing and analyzing map smoothness both conceptually and in challenging practical settings.

==> macros.tex <==
% \newcommand{\Aa}{\mathcal{A}}

% \newcommand{\ZZ}{\mathbb{Z}}
% \newcommand{\CC}{\mathbb{C}}
% \newcommand{\RR}{\mathbb{R}}
% \newcommand{\EE}{\mathbb{E}}
% \newcommand{\PP}{\mathbb{P}}
% \newcommand{\Zz}{\mathcal{Z}}
% \newcommand{\Kk}{\mathcal{K}}
% \newcommand{\Ww}{\mathcal{W}}
% \newcommand{\Vv}{\mathcal{V}}
% \newcommand{\Nn}{\mathcal{N}}
% \newcommand{\NN}{\mathbb{N}}
% \newcommand{\Hh}{\mathcal{H}}
% \newcommand{\Bb}{\mathcal{B}}
% \newcommand{\Ee}{\mathcal{E}}
% \newcommand{\Cc}{\mathcal{C}}
% \newcommand{\Gg}{\mathcal{G}}
% \newcommand{\Ss}{\mathcal{S}}
% \newcommand{\Pp}{\mathcal{P}}
% \newcommand{\Ff}{\mathcal{F}}
% \newcommand{\Xx}{\mathcal{X}}
% \newcommand{\Yy}{\mathcal{Y}}
% \newcommand{\Mm}{\mathcal{M}}
% \newcommand{\Ii}{\mathcal{I}}
% \newcommand{\Dd}{\mathcal{D}}
% \newcommand{\Ll}{\mathcal{L}}
% \newcommand{\Tt}{\mathcal{T}}
% \newcommand{\Oo}{\mathcal{O}}
% \newcommand{\Uu}{\mathcal{U}}
% \newcommand{\tht}{\theta}
% \newcommand{\Tht}{\Theta}
% \newcommand{\eps}{\varepsilon}
% \newcommand{\al}{\alpha}
% \newcommand{\be}{\beta}
% \newcommand{\de}{\delta}
% \newcommand{\De}{\Delta}
% \newcommand{\gam}{\gamma}
% \newcommand{\Sig}{\Sigma}
% \newcommand{\sig}{\sigma}
% \newcommand{\lb}{\lambda}
% \newcommand{\Lb}{\Lambda}
% \newcommand{\vphi}{\varphi}
% \newcommand{\Gam}{\Gamma}


% \newcommand{\uargmin}[1]{\underset{#1}{\text{argmin}}\;}
% \newcommand{\uargmax}[1]{\underset{#1}{\text{argmax}}\;}

% \def\*#1{\mathbf{#1}}

% \newcommand{\evm}{\*\Phi^\Mm}
% \newcommand{\evn}{\*\Phi^\Nn}

% \newcommand{\inpar}[1]{\left(#1\right)}

==> sections/old_text.tex <==

% Note that is f is
% %
% For $K$-dimensional function $F\in\mathbf{R}^{n\times K}$, we can similarly measure its smoothness via Dirichlet energy by summing over all the dimensions:
% \begin{equation}
%     \mathcal{D}\big(F \,\vert\, S\big) = \text{trace}\big( F^T L^{\omega} F\big) = \big\Vert F \big\Vert_{L^{\omega}}^2.
% \end{equation}
% A natural choice of $L^{\omega}$ is the cotangent weight matrix $W$ of shape $S$~\cite{RHM}.

% Dirichlet energy can also be extended to measure the smoothness of a given pointwise map $\Pi_{ij}$.
% %
% Specifically, one trivial formulation would be measure the Dirichlet energy on the pull-back shape $\tilde{S}_{i}$:
% \begin{equation}
%     \mathcal{D}\big(\Pi_{ij}\big) = \big\Vert \Pi_{ij}X_j\big\Vert_{W_i}^{2},
% \end{equation}
% where $X_j$ is the vertex coordinates of shape $S_j$, and $W_i$ is the cotangent weight matrix of shape $S_i$.
%





%
%and show how closely related they are to each other by reformulating them using common notations. We finally show that these multiple variants can be compared coherently within a single framework, for which we release a unified code.

%
%
%is a highly classical problem in computer graphics and for a reason : most shape analysis tools rely on the existence of underlying correspondences between some pairs of shapes. This makes the acquisition or computation of reliable and high-quality dense correspondences a key area of research. How to assess the quality of a map between two non-isometric surfaces remain however an open question for which multiple answers coexists, since no single metric allows to unilaterally discriminate between a right and a wrong map. One of the standard way to evaluate correspondences is to inspect the agreement between known correspondences between some points - or landmarks - and the computed ones. This however requires some prior knowledge about the two shapes, namely human supervision to place landmarks, and can remain a poor criteria in case of scarce landmarks as correspondences could be chaotic outside of the immediate neighborhood of the landmarks. A maybe more natural way to ensure that a map is reliable is \emph{smoothness}, that is the fact local neighborhoods are mapped into local neighborhoods. The smoothness criteria is universally accepted as a necessary condition for high-quality maps, but remain however quite qualitative as it is cumbersome to define local neighborhoods for discrete surfaces. We here argue that a smooth map, even  slightly approximate on landmarks preservation, can often appear more useful for analysis than precise but erratic one.
%
%
%A first reasonable approach to obtain smooth correspondences between two shapes lies in the smooth deformation of one shape into another. Since deformation fields are more intuitive to deal with than correspondences, these techniques allow to enforce explicit design choice of deformations through closed-form expressions or even differential equations, which then intrinsically enforce smoothness . Eventually these methods only rely on the extrinsic geometry of the shapes and are prone to fail in the absence of guidance in the form of landmarks preservation or pre-alignment of shapes.
%Another line of work uses the Dirichlet energy of a map as a criterion for smoothness and seeks to obtain often both bijective and smooth map by solving a constrained optimization problem which, with a right initialization, can lead to great results but remain very slow. Finally the domain of functional maps has been developed as a flexible way to perform shape matching using low pass filtering to obtain correspondences, which enforces some form of smoothness by definition. These methods have shown great results in computing dense correspondence from poor initialization, but the lack of an explicit regularization towards smooth maps in the algorithms can make the method fail in highly non-isometric scenarios. More related to our work is the Smooth Shells algorithm, which combines the functional map framework and the smooth deformation field approach in a unified algorithm. It however remains unclear which term enforces smoothness in this approach, which we will here investigate.
%
%
%In this work, we design an algorithm which allows to naturally introduce smoothness in the functional map framework, and enables to robustly produce smooth maps from noisy inputs. We also investigate multiple methods for smoothness and show how closely related they are to each other by reformulating them using common notations. We finally show that these multiple variants can be compared coherently within a single framework, for which we release a unified code.
%

%t o Multiple works have tried to enforce smoothness of correspondences, firstly through the use of a smooth deformation fields, often via an explicit closed-form expression of the deformation which eventually guarantees smoothness. These methods do however often require guidance in the form of landmarks preservation or initial alignment. Some other work have worked directly on optimizing correspondence matrices in order the reduce their Dirichlet energy which leads to great results, although very slow and reliant on initialization. Functional correspondences have also been developed as a fast and flexible way to perform shape matching, and while their multi-scale approach have shown good results on smoothness, the lack of an explicit regularization towards smooth maps in their formulation make some algorithm fail in non-isometric scenarios. More related to our work is the method developed in Smooth Shells, which leverages on both the flexibility of functional maps and a somewhat constrained deformation fields in order to obtain smooth and reliable correspondences. The smoothness regularization is however hidden within a search-space reduction and remain hard to tune.
%Our contribution is twofold : 1) We bring together these multiple approaches into a common formulation, 2) We create a very flexible framework which generalizes and extend these methods which allows to compute smooth correspondences between non-isometric shapes.


\subsection{Smoothness Reformulation}
\robin{This is a previous version of the section above.}
We first demonstrate that different smoothness terms introduced in the previous work can be reformulated in a consistent manner, i.e., as a Dirichlet energy defined on a map or a deformation field.
%
For example, though the ultimate goal is to wrap the source shape $\Ss_1$ onto a target shape $\Ss_2$ which is encoded as a deformation field $\*D$, nICP implicitly maintain a pointwise map $\Pi_{12}$ from $\Ss_1$ to $\Ss_2$, such that $\*D\circ X_1 \simeq \Pi_{12}X_2$, where $\*D\circ X_1$ gives the updated vertex positions after applying the per-vertex affine transformation $\*D$, and $\Pi_{12}X_2$ gives the expected vertex position on the target shape. nICP then proposes a smoothness regularizer posed on the deformation field $\*D$:
\begin{equation}
    E_{\text{nicp}}^{\text{smooth}}({\*D}) = \sum_{(v_i, v_j)\in\Ee(\Ss_1)} \big\Vert D_i - D_j \big\Vert_F^2 = \big\Vert \*D \big\Vert_{W_1},
\end{equation}
%
where $D_i\in\*D$ is a to-be-determined affine transformation defined on vertex $v_i$. We can see that the original smoothness term can be reformulated as the Dirichlet energy on $\*D$ w.r.t. the graph Laplacian (with uniform weights) $W_1$ of shape $\Ss_1$.


ARAP proposes a simple energy to enforce local rigidity for shape deformation:
\begin{align}
    E_{\text{arap}}(R, q) &= \sum_{(v_i, v_j)\in\Ee(\Ss_1)} w_{ij} \big\Vert (q_i - q_j) - R_i (v_i - v_j) \big\Vert_F^2
\end{align}
where in the context of shape matching, $q_i$ is the position of the corresponding vertex on the target shape $\Ss_2$ w.r.t. the vertex $v_i$ on the source shape $\Ss_1$, and $R_i$ is an auxiliary variable defined on vertex $v_i$ and constrained to be a rotation matrix to enforce local rigidity. 
%
We can see that the ARAP energy can be decomposed into two main components including a smoothness term and a rigidity term: 
\begin{align}
    E_{\text{arap}}(R, q) & = E_{\text{arap}}^{\text{smooth}}(q) + 2E_{\text{arap}}^{\text{rigid}}(R, q) + \text{const.}\\
    E_{\text{arap}}^{\text{smooth}}(q) & = \sum_{(v_i, v_j)\in\Ee(\Ss_1)} w_{ij} \big\Vert q_i - q_j\big\Vert_F^2,\\
    E_{\text{arap}}^{\text{rigid}}(R, q) & = \sum_{(v_i, v_j)\in\Ee(\Ss_1)} w_{ij} \big\Vert (q_i - q_j)^T R_i (v_i - v_j)\big\Vert_F^2.
\end{align}
%
We are particularly interested in the smoothness component, which can be easily reformulated as the Dirichlet energy on the mapped vertex positions $Q$, i.e., $E_{\text{arap}}^{\text{smooth}} = \big\Vert Q \big\Vert_{W_1}$.
%
%
SmoothShells also adopts the ARAP smoothness energy in its formulation. However, the mapped vertex positions in SmoothShells are obtained via a projected deformation (displacement) field.


RHM proposes to minimize the Dirichlet energy together with a bijectivity term to avoid trivial solution for shape matching. Specifically, RHM proposes the following smoothness term:
\begin{equation}
    E_{\text{rhm}}^{\text{smooth}} (\Pi_{12}) = \big\Vert \Pi_{12}\tilde{X}_2\big\Vert_{W_1}, 
\end{equation}
where $\tilde{X}_2$ is a high-dimensional embedding of the geodesic distances of shape $S_2$ vis MDS~\cite{cox2008multidimensional}.






%--------------------------------- old version of formulation
In our formulation, we consider the functional maps $C_{ij}$ and the pointwise maps $\Pi_{ij}$ from \emph{both} directions of the input shapes $\Ss_1$ and $\Ss_2$, where index $i,j \in \{0,1\}$ indicates the map direction.
%
For simplicity of notation, we denote $E(C) = E(C_{12}) + E(C_{21})$ ( or $E(\Pi) = E(\Pi_{12}) + E(\Pi_{21})$) for a given energy function $E(\cdot)$ defined on functional (or pointwise) maps where both directions are taken into consideration.


\paragraph*{Bijectivity on Functional Maps} We have the bijectivity energy on functional maps defined as:
\begin{equation}\begin{split}
    E_{\text{bi}}(C) &=  E_{\text{bi}}\big(C_{12}, C_{21}\big) + E_{\text{bi}}\big(C_{21}, C_{12}\big)\\
    &= \big\Vert C_{12} C_{21} - I_{k_2} \big\Vert_F^2 + \big\Vert C_{21} C_{12} - I_{k_1} \big\Vert_F^2,
\end{split}\end{equation}
where $I_k$ is a $k\times k$ identity matrix.
Recall that to minimize this energy in the proper functional map space using the discrete solver (Sec.~\ref{sec:background:discrete_solver}), we iteratively solve for the functional maps and the underlying pointwise maps by optimizing the following unconstrained energy:
\begin{equation}\label{eq:bijectivity}
    E_{\text{bijectivity}}(C, \Pi) = w_1 E_{\text{bi}}\big(C, \Pi\big) + w_2 E_{\text{couple}}\big(C, \Pi\big),
\end{equation}
%
where the coupling term is defined in Eq.~\eqref{eq:coupling}.

\paragraph*{Smoothness on Pointwise Maps} We then adopt the Dirichlet energy discussed in Sec.~\ref{sec:background:dirichlet} to regularize the smoothness of pointwise maps: $E_{D}(\Pi) = E_{D}(\Pi_{12}) + E_D(\Pi_{21})$ where the Dirichlet energy $E_D(\cdot)$ is defined in Eq.~\eqref{eq:Dirichlet pull back}. 
%
One can easily observe that it is complicated to solve $\Pi$ from the sum of the bijectivity term (with coupling terms) and the smoothness terms since different norms are used.
We therefore introduce auxiliary variables $Y_{ij}$ to construct a coupling term in the \emph{spatial} domain similarly to the coupling term defined in the \emph{spectral} domain as proposed in the discrete solver (see Eq.~\eqref{eq:coupling}).
Specifically, the coupling term in the spatial domain enforces $Y_{ij}$ to be close to the pull-back shapes $\Pi_{ij}X_j$. We then have the smoothness energy $E_{\text{smooth}}(\Pi, Y)$ defined as:
\begin{equation}\label{eq:smooth}
    E_{\text{smooth}}\big(\Pi_{ij}, Y_{ij}\big) = w_3 E_D\big( Y_{ij}\big) + w_4 \big\Vert Y_{ij} - \Pi_{ij} X_j\big\Vert_{A_i}.
\end{equation}


\paragraph*{Total Energy} Eventually, our global energy is simply set as the sum of the bijectivity on functional maps~\eqref{eq:bijectivity} and the new smoothness energy~\eqref{eq:smooth}, which results in a 3-variable optimization problem:
\begin{equation}
    E_{\text{ours}}(\Pi, C, Y) = E_\text{smooth}(\Pi, Y) + E_{\text{biject}}(\Pi, C)
\end{equation}




\begin{table}[!t]
\centering
\caption{\textbf{Accuracy} on \textsc{DeformThings4D-Matching}}
\label{tab:append:deform_acc}
\footnotesize
{\def\arraystretch{1.05}\tabcolsep=0.36em
\begin{tabular}{ccccccc}\toprule[0.8pt]
\multirow{2}{*}{methods} & \multicolumn{4}{c}{\textbf{\textit{near-isometric}}} & \textbf{\textit{partial}} & \textbf{\textit{non-iso}} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
 & \textsc{Zlorp} & \textsc{Drake} & \textsc{Mannequin} & \textsc{Ninja} & \textsc{Prisoner} & \textsc{Zombie}  \\ \midrule[0.8pt]
ARAP & $11.22$ & $9.04$  & $8.10$  & $9.88$  & $19.91$  & $14.83$    \\
NICP  & $7.29$ & $7.07$  & $4.61$  & $5.25$  & $21.18$  & $11.95$  \\
RHM & $3.70$ & $5.63$  & $3.94$  & $5.46$  & $18.85$  & $11.00$    \\
Shells & $3.25$ & $7.78$  & $4.11$  & $4.73$  & $20.27$  & $10.32$    \\ 
ZO & $3.43$ & $5.74$  & $3.33$  & $4.61$  & $20.59$  & $13.71$    \\
DO & $3.26$ & $5.95$  & $3.64$  & $5.10$  & $19.59$  & $16.53$    \\ \midrule[0.8pt]
Ours & $3.72$ & $6.93$  & $4.18$  & $4.80$  & $19.81$  & $9.71$    \\
Ours$^*$ & $3.89$ & $7.25$  & $4.22$  & $5.16$  & $19.62$  & $8.31$    \\ \bottomrule[0.8pt]
\end{tabular}}
\end{table}





\begin{table}[!t]
\caption{\textbf{Bijectivity} on \textsc{DeformThings4D-Matching}}\label{tab:append:deform_biject}
\centering
\footnotesize
{\def\arraystretch{1.05}\tabcolsep=0.38em
\begin{tabular}{ccccccc}\toprule[0.8pt]
\multirow{2}{*}{methods} & \multicolumn{4}{c}{\textbf{\textit{near-isometric}}} & \textbf{\textit{partial}} & \textbf{\textit{non-iso}} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
 & \textsc{Zlorp} & \textsc{Drake} & \textsc{Mannequin} & \textsc{Ninja} & \textsc{Prisoner} & \textsc{Zombie}  \\ \midrule[0.8pt]
ARAP & $11.93$ & $7.25$  & $7.69$  & $10.42$  & $21.71$  & $11.18$    \\
nICP & $3.63$ & $2.73$  & $2.58$  & $2.49$  & $7.17$  & $4.71$    \\
RHM & $1.42$ & $1.84$  & $1.82$  & $1.94$  & $2.81$  & $3.24$    \\
Shells & $1.67$ & $2.16$  & $2.22$  & $2.23$  & $3.56$  & $3.71$    \\
ZO & $2.14$ & $4.05$  & $1.37$  & $3.99$  & $21.19$  & $10.11$    \\
DO & $1.27$ & $1.55$  & $1.63$  & $1.46$  & $2.26$  & $2.52$   \\ \midrule[0.8pt]
Ours & $1.77$  & $2.12$  & $2.30$  & $2.25$  & $3.60$  & $3.74$   \\
Ours$^*$  & $1.76$ & $2.15$  & $2.35$  & $2.30$  & $3.49$  & $3.78$   \\ \bottomrule[0.8pt]
\end{tabular}
}
\end{table}
% tosca - include man v.s. woman
\begin{table}[]
\centering
\caption{Caption}
\label{tab:res:tosca}
\footnotesize
\begin{tabular}{c|cccc}
& Accuracy & Bijectivity & Smoothness & Coverage \\
Init & $5.86$  & $5.87$  & $1.71$ & $34.37$ \% \\
ARAP & $5.73$  & $6.33$  & $0.82$ & $53.59$ \% \\
nICP & $5.60$  & $2.82$  & $1.03$ & $47.57$ \% \\
RHM & $4.55$  & $1.52$  & $1.18$ & $58.45$ \% \\
Shells & $8.54$  & $5.04$  & $1.02$ & $44.01$ \% \\
ZoomOut & $8.32$  & $5.54$  & $3.92$ & $61.22$ \% \\
DiscreteOpt & $8.74$  & $1.55$  & $3.59$ & $57.76$ \% \\
Ours & $5.23$  & $2.47$  & $1.04$ & $47.69$ \% \\
Ours$^*$ & $7.85$  & $2.92$  & $1.06$ & $43.81$ \% \\
\end{tabular}
\end{table}




\begin{table}[!t]
\centering
\caption{\textbf{Coverage} on \textsc{DeformThings4D-Matching}}\label{tab:append:deform_cov}
\footnotesize
{\def\arraystretch{1.05}\tabcolsep=0.38em
\begin{tabular}{ccccccc}\toprule[0.8pt]
\multirow{2}{*}{methods} & \multicolumn{4}{c}{\textbf{\textit{near-isometric}}} & \textbf{\textit{partial}} & \textbf{\textit{non-iso}} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
 & \textsc{Zlorp} & \textsc{Drake} & \textsc{Mannequin} & \textsc{Ninja} & \textsc{Prisoner} & \textsc{Zombie}  \\ \midrule[0.8pt]
ARAP  & $28$\% & $37$\%  & $36$\%  & $34$\%  & $22$\%  & $29$\%  \\
NICP & $38$\% & $50$\%  & $53$\%  & $53$\%  & $20$\%  & $30$\%    \\
RHM & $64$\%  & $60$\%  & $60$\%  & $60$\%  & $45$\%  & $47$\%   \\
Shells & $61$\%  & $55$\%  & $56$\%  & $57$\%  & $39$\%  & $43$\%   \\
ZO & $72$\%  & $70$\%  & $71$\%  & $71$\%  & $59$\%  & $60$\%   \\
DO & $68$\% & $66$\%  & $65$\%  & $66$\%  & $55$\%  & $55$\%    \\ \midrule[0.8pt]
Ours & $59$\% & $55$\%  & $54$\%  & $56$\%  & $37$\%  & $41$\%    \\
Ours$^*$ & $59$\% & $55$\%  & $53$\%  & $55$\%  & $38$\%  & $43$\%    \\ \bottomrule[0.8pt]
\end{tabular}}
\end{table}


\begin{table}[!t]
\centering
\caption{\textbf{Smoothness} on \textsc{DeformThings4D-Matching}}
\label{tab:append:deform_smooth}
\footnotesize
{\def\arraystretch{1.05}\tabcolsep=0.38em
\begin{tabular}{ccccccc}\toprule[0.8pt]
\multirow{2}{*}{methods} & \multicolumn{4}{c}{\textbf{\textit{near-isometric}}} & \textbf{\textit{partial}} & \textbf{\textit{non-iso}} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
 & \textsc{Zlorp} & \textsc{Drake} & \textsc{Mannequin} & \textsc{Ninja} & \textsc{Prisoner} & \textsc{Zombie}  \\ \midrule[0.8pt]
ARAP & $2.33$ & $2.99$  & $2.21$  & $2.24$  & $3.02$  & $2.10$    \\
NICP  & $4.14$ & $5.15$  & $2.59$  & $2.90$  & $10.49$  & $4.58$   \\
RHM   & $2.88$ & $3.92$  & $2.78$  & $3.07$  & $10.05$  & $4.72$   \\
Shells & $3.22$ & $4.68$  & $3.77$  & $4.56$  & $14.04$  & $7.13$    \\
ZO & $3.05$ & $5.03$  & $2.51$  & $4.22$  & $24.80$  & $15.76$    \\
DO  & $3.23$ & $5.30$  & $3.77$  & $4.69$  & $21.10$  & $16.09$   \\ \midrule[0.8pt]
Ours & $2.85$ & $3.70$  & $2.81$  & $3.05$  & $9.89$  & $4.54$    \\
Ours$^*$ & $2.66$  & $3.83$  & $2.47$  & $2.77$  & $8.96$  & $3.78$    \\ \bottomrule[0.8pt]

\end{tabular}}
\end{table}




\begin{table}[]
    \centering
    \begin{tabular}{c|ccc}
     & Accuracy & Bijectivity & Smoothness\\\hline
    ZoomOut & $83.42$  & $56.85$ & $15.26$\\
    Discrete Opt & $86.90$ & $15.22$ & $15.46$\\
    \hline
    Ours exact & $50.03$ & $24.76$ & $5.33$\\
    Ours proj & $76.88$ & $29.34$ & $5.64$\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> sections/sec_smoothness_old.tex <==
%\robin{Add references to the meta-algo / smoothness term here for coherence}
In this section, we review and standardize some popular formulations for smoothness introduced in different methods, including ICP~\cite{ICP}, non-rigid ICP (nICP)~\cite{nicp}, as-rigid-as-possible (ARAP)~\cite{arap}, reversible harmonic maps (RHM)~\cite{RHM}, and Smooth Shells~\cite{smoothshells}. For each of these methods, we seek to highlight the smoothness term in the form of the Dirichlet energy of either a map or a deformation. In addition to the harmonization of the formulations, the different energy terms and solvers can later be introduced in our Smoothness-promoting Discrete Solver in a straightforward way.


%While the Dirichlet energy defines a measure of the distortion induced by a map, we highlight that mapping all vertices in $\Ss_1$ to a single vertex in $\Ss_2$ leads to a $0$ energy, as seen by setting $f(x_i)=y$ for some $y\in\Ss_2$ and all $x_i\in\Ss_1$ in equation~\eqref{eq:bg:dirichlet_def}. 
%

% Multiple works have tried to enforce smoothness when computing shape correspondneces

% Smoothness has been taken into consideration during shape correspondences computation in previous work.
% In this section, we provide a unified framework focusing on Dirichlet energy to analyze the smoothness formulation introduced in different methods, including non-rigid ICP (nICP)~\cite{nicp}, as-rigid-as-possible (ARAP)~\cite{arap}, reversible harmonic maps (RHM)~\cite{RHM}, and smooth shells~\cite{smoothshells}.

\subsection{Smoothness Reformulation}
We divide the different methods into two groups: those optimizing for smooth \textit{deformations} and those operating with pulled-back vertices, as discussed above.

%The fact of the Dirichlet energy is globally minimized by trivial maps suggests that when enforcing smoothness using Dirichlet energy we need additional regularization through either search-space restriction, reduction of the variability or even both as discussed in the following. 
%We refer the reader to Appendix~\ref{sec:appendix:smooth} for more details on the reformulation or slight modifications of different methods, or abuse of notations which might be used here. 

\paragraph*{Using Deformations.} A direct way to enforce smoothness in a matching pipeline is to ensure that the \emph{deformation} from one shape to the other is smooth, where the smoothest existing kind of transformation are translations and possibly rigid transformations. Two main methods coexist to try to enforce this property: (1) designing a specific family of deformations, or (2) reducing the \textit{Dirichlet energy} of the deformation.
A natural energy to minimize in order to compute deformation-driven correspondence is therefore :
\begin{equation}\label{eq:base equation deformation}
    E_{\text{deform}}(\Pi_{12}, \*D) = E_D(\*D) + \|\Pi_{12} X_2 - \*D(X_1)\|^2_{A_1},
\end{equation}
which contains both the Dirichlet energy of the deformation and a coupling term between the deformed vertices of $\Ss_1$ and the pulled-back vertices using current point-wise map. 
This energy can be solved in an alternating manner between $\Pi_{12}$ and $\*D$, constraining $\*D$ to lie in some specific space.

Both ICP~\cite{ICP} and nICP~\cite{nicp} seek to minimize $E_{\text{deform}}$, each using a different search space for $\*D$. On the one hand ICP restricts $\*D$ to be a rigid transformation, which sets $E_D(\*D)$ to $0$. On the other hand, nICP designs $\*D$ as an affine transformation on each vertex. Some slight modification have been done and we refer the reader to Appendix~\ref{sec:appendix:smooth} for details.%, which implies a slight modification of the formulation as this transformation is not linear on vertices per se (see appendix for more details). 

Smooth Shells~\cite{smoothshells} models the deformation as a simple per-vertex translation seen as a function $\Ss_1\to\RR^3$, then restricted to lie in the spectral basis of size $K$. Energy $E_{\text{deform}}$ is however further regularized using a alignment term from ARAP~\cite{arap}:
%
Instead of computing the map $\Pi_{12}$, ARAP directly predicts the coordinates of the pulled-back vertices $Y_{12} =\Pi_{12}X_2$ by constraining the deformation to be locally rigid. The deformation is denoted as $\*R$ to simplify some next equations, and locally acts as a rotation $R_i$ around $x_i$. As seen in the appendix, the ARAP energy can be rewritten as:
\begin{equation}\label{eq:smooth:arap energy}
    E_{\text{arap}}(\*R, Y_{12}) = E_D(Y_{12}) - 2E_{\text{arap}}^{\text{rigid}}(\*R, Y_{12})  + \text{const.}
\end{equation}
where $E_{\text{arap}}^{\text{rigid}}$ measures the alignment between the estimated edges and the rotated ones :
\begin{equation}
    E_{\text{arap}}^{\text{rigid}}(\*R, Y) =  \sum_{(i, j)\in\Ee(\Ss_1)} w_{ij} \left\langle Y_i - Y_j,\ R_i (x_i - x_j)\right\rangle
\end{equation}
%
The ARAP energy Eq.~\eqref{eq:smooth:arap energy} considers the estimated Dirichlet energy $E_D(Y_{12})$ but pushes towards a locally rigid map. However since $Y_{12}$ is not constrained to remain on the surface of $\Ss_2$, the method remains reliant on pre-existing landmarks.

Inspired by this, smooth shells~\cite{smoothshells} also enforces its deformation field $\*D$ to be close to a rigid deformation via:
\begin{equation}
    E_{\text{shells}}(\Pi_{12}, \*D, \*R) = E_{\text{def}}(\Pi_{12}, \*D) - 2 E_{\text{arap}}^{\text{rigid}}(\*R, X_1 +\*D),
\end{equation}
%
where the ARAP term again pushes towards a locally rigid transformation. This energy can also be obtained by summing the ARAP energy term Eq.~\eqref{eq:smooth:arap energy} and the coupling term from Eq.~\eqref{eq:base equation deformation}. Additionally, smooth shells use a smoothed version of the vertex coordinates, given by a similar smoothing as for $\*D$. Note that terms including normals or spectral alignment have been ignored. %One particularity of smooth shells is that each iterations used a smoothed version of the vertex coordinates, obtained by the same projection in the spectral basis as $\*D$. Other terms in the optimization include normals and spectral alignment are discarded are they are not introduced specifically for smoothness.

\paragraph*{Using Pull-Back Shapes} Another line of work~\cite{RHM} directly minimizes the Dirichlet energy of a map without deformation design. To avoid making the map collapse the authors look for bijective maps with the lowest possible Dirichlet energy. Vertices of the pull-back shape $\Pi_{ij}X_j$ for $(i,j)\in\left\{(1,2), (2,1) \right\}$ are again estimated via an auxiliary variable $Y_{ij}$ and the energy reads as the sum on both directions of $E_{\text{rhm}}^{\text{half}}$ with :
\begin{equation}
\begin{split}
    E_{\text{rhm}}^{\text{half}}\left(\Pi_{ij},\Pi_{ji},Y_{ij},Y_{ji}\right) =&\ E_D(Y_{ij}) + E_{\text{rhm}}^{\text{bij}}(\Pi_{ji}, Y_{ij})\\ &+ E_{\text{rhm}}^{\text{couple}}(\Pi_{ij}, Y_{ij})
\end{split}
\end{equation}
where we recognize the Dirichlet energy of the estimated map $E_D(Y_{ij})$, and two terms $E_{\text{rhm}}^{\text{bij}}$ and $E_{\text{rhm}}^{\text{couple}}$ which respectively enforce bijectivity and coupling: 
\begin{align}
    E_{\text{rhm}}^{\text{bij}}(\Pi_{ji}, Y_{ij}) &= \big\Vert \Pi_{ji}Y_{ij} - X_j\big\Vert^2_{A_j} \\
    E_{\text{rhm}}^{\text{couple}}(\Pi_{ij}, Y_{ij}) &= \big\Vert Y_{ij} - \Pi_{ij}X_j\big\Vert_{A_i}
\end{align}
This formulation leads to a slow iterative solver which can obtain to great results given an already good initialization. Additionally, the authors use a high-dimensional embedding for the vertices obtained via MDS~\cite{cox2008multidimensional} which mimics the geodesic distance.


\paragraph*{Summary} We can summarize the differences between smoothness formulation in the methods discussed above via the search-space restriction (see Table~\ref{tab:search space recap}). 
Specifically, nICP associates a $3\times 4$ affine transformation to each vertex, which leads to a search space of size $n_1\times 3 \times 4$, with $n_1$ is the number of vertices on the source shape $\Ss_1$.
%
In contrast SmoothShells encode the mesh deformation by a vertex-wise translation in $\RR^3$, restricted to lie for each axis on the spectral basis of size $k$, leading to a search space of $K \times 3$.
%
Both ARAP and RHM have Dirichlet energy defined on the pull-back shapes to improve smoothness with different embeddings.
Specifically, ARAP uses extrinsic embeddings, i.e., the original shape vertex positions, to construct pull-back shapes.
As a comparison, RHM uses intrinsic embeddings, i.e., the high-dimensional Euclidean embeddings that approximate the geodesic distances, to construct intrinsic pull-back shapes.


\subsection{Incorporating smoothness terms in \robin{Find a nice name}}

All 

==> tables/tb_res_deform_smooth.tex <==
\footnotesize
{\def\arraystretch{1}\tabcolsep=0.32em
\begin{tabular}{ccccccc}\toprule[0.8pt]
\multirow{2}{*}{methods} & \multicolumn{4}{c}{\textbf{\textit{near-isometric}}} & \textbf{\textit{partial}} & \textbf{\textit{non-iso}} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
 & \textsc{Zlorp} & \textsc{Drake} & \textsc{Mannequin} & \textsc{Ninja} & \textsc{Prisoner} & \textsc{Zombie}  \\ \midrule[0.8pt]
 Init & $2.74$ & $3.23$  & $4.09$  & $2.79$  & $5.57$  & $3.18$   \\ \midrule[0.5pt]
ARAP & \cellcolor{tabblue!25} $0.71$ & \cellcolor{tabblue!25} $0.74$  & \cellcolor{tabblue!25} $0.76$  &\cellcolor{tabblue!25} $0.73$  & \cellcolor{tabblue!25} $0.68$  & \cellcolor{tabblue!25} $0.67$    \\
nICP & $1.41$ & $1.16$  & \cellcolor{tabblue!25}$0.89$  & \cellcolor{tabblue!25}$0.97$  & $4.36$  & \cellcolor{tabblue!25}$1.54$    \\
%RHM & $0.89$ & $1.04$  & $0.95$  & $1.01$  & \cellcolor{tabblue!25} $3.32$  & $1.60$    \\
Shells & $0.98$ & $1.29$  & $1.24$  & $1.38$  & $5.64$  & $2.56$    \\ \midrule[0.5pt]
ZO & $1.04$ & $1.08$  & $0.88$  & $1.29$  & $13.70$  & $6.12$    \\
DO & $0.99$ & $1.19$  & $1.27$  & $1.45$  & $9.09$  & $5.30$    \\ \midrule[0.5pt]
Ours & $0.92$ & \cellcolor{tabblue!25} $0.99$  & $0.96$  & $1.00$  & $3.93$  & $1.58$    \\
Ours$^*$ & \cellcolor{tabblue!25}$0.89$ & $1.04$  & $0.95$  & $1.01$  & \cellcolor{tabblue!25} $3.32$  & $1.60$    \\ \bottomrule[0.8pt]
%Ours$^*$ &\cellcolor{tabblue!20} $0.83$ & $1.00$  & \cellcolor{tabblue!25} $0.84$  & \cellcolor{tabblue!25} $0.92$  & $3.35$  & \cellcolor{tabblue!25} $1.32$    \\ \bottomrule[0.8pt]
\end{tabular}}


